Bayesian Posterior Interval Calibration to Improve the Interpretability of Observational Studies

Observational healthcare data offer the potential to estimate causal effects of medical products on a large scale. However, the confidence intervals and p-values produced by observational studies only account for random error and fail to account for systematic error. As a consequence, operating characteristics such as confidence interval coverage and Type I error rates often deviate sharply from their nominal values and render interpretation impossible. While there is longstanding awareness of systematic error in observational studies, analytic approaches to empirically account for systematic error are relatively new. Several authors have proposed approaches using negative controls (also known as "falsification hypotheses") and positive controls. The basic idea is to adjust confidence intervals and p-values in light of the bias (if any) detected in the analyses of the negative and positive control. In this work, we propose a Bayesian statistical procedure for posterior interval calibration that uses negative and positive controls. We show that the posterior interval calibration procedure restores nominal characteristics, such as 95% coverage of the true effect size by the 95% posterior interval.

==> tikz-bayesnet/README <==
BayesNet
========

TikZ library for drawing Bayesian networks, graphical models and (directed) factor
graphs in LaTeX.

Contents
--------

Provides the following node styles:

* :code:`latent`

* :code:`obs`

* :code:`det`

* :code:`const`

* :code:`factor`

* :code:`plate`

* :code:`gate`

Provides the following commands (note that any of the arguments can be
empty):

* :code:`\factor [options] {name} {caption} {inputs} {outputs}`

* :code:`\plate [options] {name} {fitlist} {caption}`

* :code:`\gate [options] {name} {fitlist} {inputs}`

* :code:`\vgate {name} {fitlist-left} {caption-left} {fitlist-right}
  {caption-right} {inputs}`

* :code:`\hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
  {caption-bottom} {inputs}`

* :code:`\edge [options] {inputs} {outputs}`

* :code:`\factoredge [options] {inputs} {factors} {outputs}`

Usage
-----

Install the package by copying tikzlibrarybayesnet.code.tex to your
LaTeX system or copy the file into projects that are using it.  To use
the library in your LaTeX file

.. code-block:: python

   \usepackage{tikz}
   \usetikzlibrary{bayesnet}

Compile the LaTeX example:

.. code-block:: none

   pdflatex example.tex

and see the resulting PDF file example.pdf.

Example
-------

.. figure:: http://i.imgur.com/CzNyk.png
   :align: center
   :alt: Bayesian network.

   PCA model as a Bayesian network and a directed factor graph.

.. figure:: http://i.imgur.com/CBZqL.png
   :align: center
   :alt: Citation influence model

   Directed factor graph of the citation influence model.


Related projects
----------------

This library is derived from a technical report "Directed Factor Graph
Notation for Generative Models" and the accompanying TikZ macros by
Laura Dietz 2010 (http://people.cs.umass.edu/~dietz/).

GraphViz (http://www.graphviz.org/) is a more general open source
graph visualization software.  It uses DOT file format to describe the
structure of the graph.  The DOT file can be converted to LaTeX using
:code:`dot2tex` (http://www.fauskes.net/code/dot2tex/).

UAI (http://graphmod.ics.uci.edu/uai08/FileFormat) is a simple text
file format to describe Markov networks. The UAI file format can be
converted to DOT file format using :code:`uai2dot`
(https://github.com/drewfrank/uai2dot).

License
-------

| Copyright (C) 2010-2011 Laura Dietz
| Copyright (C) 2012 Jaakko Luttinen jaakko.luttinen@aalto.fi

This work may be distributed and/or modified under the conditions of
the LaTeX Project Public License, either version 1.3 of this license
or (at your option) any later version.  The license is in the file
LICENSE_LPPL and the latest version of this license is in
http://www.latex-project.org/lppl.txt and version 1.3 or later is part
of all distributions of LaTeX version 2005/12/01 or later.

This work is free software: you can redistribute it and/or modify it
under the terms of the GNU General Public License as published by the
Free Software Foundation, either version 3 of the License, or (at your
option) any later version.  This work is distributed in the hope that
it will be useful, but WITHOUT ANY WARRANTY; without even the implied
warranty of MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See
the GNU General Public License for more details.  See the license in
the file LICENSE_GPL or visit <http://www.gnu.org/licenses/>.




==> tikz-bayesnet/model_citation_influence.tex <==
% model_citation_influence.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Citation influence model
% Cite this model as 
% Laura Dietz, Steffen Bickel, Tobias Scheffer. 
% Unsupervised Prediction of Citation Influences. 
% In: Proceedings of International Conference on Machine Learning. 2007

%\beginpgfgraphicnamed{model-citation-influence}
\begin{tikzpicture}

  % Layout the variables
  \matrix[row sep=0.5cm, column sep=1.2cm] (LDA)
  { %
    & %
    & %
    \node[latent] (gamma)  {$\gamma$} ; & %
    \node[latent] (lambda) {$\lambda$} ; & %
    \node[latent] (psi)    {$\psi$} ; %
    \\
    \\
    \node[latent] (theta)  {$\theta$} ; & %
    & %
    \node[latent] (C)      {$C$} ; & %
    \node[latent] (S)      {$S$} ; & %
    \\
    & %
    & %
    \factor       {T-f1}   {Multi} {} {}; & %
    & %
    \factor       {T-f2}   {below:Multi} {} {}; & %
    \\
    \node[latent] (T')     {$T'$} ; & %
    & %
    \node[latent] (T)      {$T$} ; & %
    \\
    \factor       {W'-f}   {Multi} {} {}; & %
    \node[latent] (phi)    {$\phi$} ; & %
    \factor       {W-f}    {Multi} {} {}; %
    \\
    \node[obs] (W')        {$W'$} ; & %
    & %
    \node[obs] (W)         {$W$} ;
    \\
  };

  % Remaining factors
  \factor[above=of T']     {T'-f}     {left:Multi} {} {}; %
  \factor[above=of theta]  {theta-f}  {left:Dir} {} {}; %
  \factor[above=of C]      {C-f}      {left:Multi} {} {}; %
  \factor[above=of S]      {S-f}      {left:Bern} {} {}; %
  \factor[above=of gamma]  {gamma-f}  {left:Dir} {} {}; %
  \factor[above=of lambda] {lambda-f} {left:Beta} {} {}; %
  \factor[above=of psi]    {psi-f}    {left:Dir} {} {}; %
  \factor[above=of phi]    {phi-f}    {left:Dir} {} {}; %

  % Hyperparameters
  \node[const, above=of theta]  (atheta)  {$\alpha_\theta$}; %
  \node[const, above=of phi]    (aphi)    {$\alpha_\phi$}; %
  \node[const, above=of gamma]  (agamma)  {$\alpha_\gamma$}; %
  \node[const, above=of lambda, xshift=-0.5cm] (alambda1)
  {$\alpha_{\lambda_\theta}$}; %
  \node[const, above=of lambda, xshift=0.5cm] (alambda2)
  {$\alpha_{\lambda_\psi}$}; %
  \node[const, above=of psi]    (apsi)    {$\alpha_\psi$}; %

  % Factor connections
  \factoredge {phi}               {W'-f}     {W'} ; %
  \factoredge {phi}               {W-f}      {W} ; %
  \factoredge {theta}             {T'-f}     {T'} ; %
  \factoredge {theta}             {T-f1}     {T} ; %
  \factoredge {psi}               {T-f2}     {T} ; %
  \factoredge {atheta}            {theta-f}  {theta} ; %
  \factoredge {gamma}             {C-f}      {C} ; %
  \factoredge {lambda}            {S-f}      {S} ; %
  \factoredge {agamma}            {gamma-f}  {gamma} ; %
  \factoredge {alambda1,alambda2} {lambda-f} {lambda} ; %
  \factoredge {apsi}              {psi-f}    {psi} ; %
  \factoredge {aphi}              {phi-f}    {phi} ; %

  % Gates
  \gate {W'-gate} {(W'-f)(W'-f-caption)} {T'} ; %
  \gate {W-gate}  {(W-f)(W-f-caption)}   {T} ; %
  \gate {T-gate}  {(T-f1)(T-f1-caption)} {C} ;
  \vgate {T-vgate} %
  {(T-gate)} {$S=0$} %
  {(T-f2)(T-f2-caption)} {$S=1$} %
  {S} ; %

  % Plates
  \plate {LDA1} { %
    (T')(T'-f)(T'-f-caption) %
    (W')(W'-gate) %
  } {$\forall w' \in c$} ; %

  \plate {LDA2} { %
    (LDA1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall c \in \mathcal{C}$} ; %

  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

  \plate {P1} { %
    (W)(W-gate) %
    (T)(T-vgate) %
    (C)(C-f)(C-f-caption) %
    (S)(S-f)(S-f-caption) %
  } {$\forall w \in d$} ;

  \plate {} { %
    (P1) %
    (gamma)(gamma-f)(gamma-f-caption) %
    (lambda)(lambda-f)(lambda-f-caption) %
    (psi)(psi-f)(psi-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> tikz-bayesnet/model_lda.tex <==
% model_lda.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Latent Diriclet allocation model

%\beginpgfgraphicnamed{model-lda}
\begin{tikzpicture}[x=1.7cm,y=1.8cm]

  % Nodes

  \node[obs]                   (X)      {$X$} ; %
  \node[latent, above=of X]    (T)      {$T$} ; %
  \node[latent, above=of T]    (theta)  {$\theta$}; %
  \node[const, above=of theta] (atheta) {$\alpha_\theta$};


  % Factors
  \factor[above=of X]     {X-f}     {Multi} {} {} ; %
  \factor[above=of T]     {T-f}     {left:Multi} {} {} ; %
  \factor[above=of theta] {theta-f} {left:Dir} {} {} ; %

  % More nodes
  \node[latent, right=of X-f] (phi)  {$\phi$}; %
  \node[const, above=of phi]  (aphi) {$\alpha_\phi$}; %

  \factor[above=of phi] {phi-f} {right:Dir} {} {} ; %

  \factoredge {theta}  {T-f}     {T} ; %
  \factoredge {atheta} {theta-f} {theta} ; %
  \factoredge {phi}    {X-f}     {X} ; %
  \factoredge {aphi}   {phi-f}   {phi} ; %

  \gate {X-gate} {(X-f)(X-f-caption)} {T}

  \plate {plate1} { %
    (X)(X-gate) %
    (T)(T-f)(T-f-caption) %
  } {$\forall 1 \leq i \leq n_d$}; %
  \plate {} { %
    (plate1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %
  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> tikz-bayesnet/model_pca.tex <==
% model_pca.tex
%
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes
  \node[obs]                               (y) {$y$};
  \node[latent, above=of y, xshift=-1.2cm] (w) {$\mathbf{w}$};
  \node[latent, above=of y, xshift=1.2cm]  (x) {$\mathbf{x}$};
  \node[latent, right=2cm of y]            (t) {$\tau$};

  % Connect the nodes
  \edge {x,w,t} {y} ; %

  % Plates
  \plate {yx} {(x)(y)} {$N$} ;
  \plate {} {(w)(y)(yx.north west)(yx.south west)} {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> tikz-bayesnet/model_pca2.tex <==
% model_pca2.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes

  % Y
  \node[obs]          (y)   {$y$}; %
  \factor[above=of y] {y-f} {left:$\mathcal{N}$} {} {} ; %

  % W and X
  \node[det, above=of y]            (dot) {dot} ; % 
  \node[latent, above left=1.2 of dot]  (w)   {$\mathbf{w}$}; %
  \node[latent, above right=1.2 of dot] (x)   {$\mathbf{x}$}; %

  % W hyperparameters
  \node[const, above=1.2 of w, xshift=-0.5cm] (mw) {$\mu_w$} ; %
  \node[const, above=1.2 of w, xshift=0.5cm]  (aw) {$\alpha_w$} ; %

  % X hyperparameters
  \node[const, above=1.2 of x, xshift=-0.5cm] (mx) {$\mu_x$} ; %
  \node[const, above=1.2 of x, xshift=0.5cm]  (ax) {$\alpha_x$} ; %

  % noise
  \node[latent, right=2.5cm of y-f]         (t)   {$\tau$}; %
  \node[const, above=of t, xshift=-0.5cm] (at)  {$\alpha_\tau$} ; %
  \node[const, above=of t, xshift=0.5cm]  (bt)  {$\beta_\tau$} ; %

  % Factors
  \factor[above=of w] {w-f} {left:$\mathcal{N}$} {mw,aw} {w} ; %
  \factor[above=of x] {x-f} {left:$\mathcal{N}$} {mx,ax} {x} ; %
  \factor[above=of t] {t-f} {left:$\mathcal{G}$} {at,bt} {t} ; %
  \factoredge {dot,t} {y-f} {y} ; %

  % Connect w and x to the dot node
  \edge[-] {w,x} {dot} ;

  % Plates
  \plate {yx} { %
    (y)(y-f)(y-f-caption) %
    (x)(x-f)(x-f-caption) %
    (dot) %
  } {$N$} ;
  \plate {} {%
    (y)(y-f)(y-f-caption) %
    (w)(w-f)(w-f-caption) %
    (dot) %
    (yx.north west)(yx.south west) %
  } {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 



==> tikz-bayesnet/tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


